Polynomial Approximation of Discounted Moments

We introduce an approximation strategy for the discounted moments of a stochastic process that can, for a large class of problems, approximate the true moments. These moments appear in pricing formulas of financial products such as bonds and credit derivatives. The approximation relies on high-order power series expansion of the infinitesimal generator, and draws parallels with the theory of polynomial processes. We demonstrate applications to bond pricing and credit derivatives. In the special cases that allow for an analytical solution the approximation error decreases to around 10 to 100 times machine precision for higher orders. When no analytical solution exists we tie out the approximation with Monte Carlo simulations.

==> Poly_processes.tex <==
This section introduces the polynomial process as it is key to our approximation. We rely heavily on \citet{cuchiero2012polynomial}, relax the definition of the process to fit our application (see \citep[Remark 2.2 (ii)]{cuchiero2012polynomial}). 
% m-polynomials defnition

%\begin{definition}
%Polynomials up to $m$ orders on space $S$ is defined as 
%\begin{equation}
%\mathcal{P}_{m}(S) \coloneqq \left\{ x \rightarrow \sum_{\mathbf{s}_{\mathbf{k}}=0}^{m} a_kx^{\mathbf{k}}, x\in S \middle| a_k\in\mathbb{R} \right\}
%\end{equation}






for bounded continuous functions [I don't think bounded, polynomials are not bounded] $f$ on domain $D$.


%where $\mathbf{k}=(k_1,k_2,\dots,k_n)\in\mathbb{N}^n$ and $x^{\mathbf{k}}=x_1^{k_1}x_2^{k_2}\dots x_n^{k_n}$, $\mathbf{s}_{\mathbf{k}}$ is defined as $\mathbf{s}_{\mathbf{k}}=k_1+k_2+\dots+k_n$. The dimension of vector here is finite, \textit{i.e.} $N<\infty$. 
%\end{definition}


% m-poly process definition
\begin{definition}
Consider a Feller process $X$ on $D$ is called $k$-polynomial process if for all $f\in\mathcal{P}_k$ it holds that
\begin{enumerate}
\item $S_tf\in\mathcal{P}_k$ for all $t\ge0$,
\item $t\rightarrow S_tf $ is continuous at $t=0$, and
\item $S_t|f(x)|<\infty$ for all $t\ge0$ and $x\in D$.
\end{enumerate}
\end{definition}

\begin{remark}
TODO: Second thing is not a consequence of the Feller property. But do we need it?
\end{remark}

\begin{remark}
TODO: How this is different from \citet{cuchiero2012polynomial}. I think we need the third bit to ensure that $f$ are in $\mathcal{D}\mathcal{A}$ (see Cuchiero's thesis definition of the generator).
\end{remark}

\begin{theorem}
For a Feller process $X$ on $D$, the following statements are equivalent:
\begin{enumerate}
\item $X$ is $k$-polynomial.
\item A matrix $A$ exists such that for all $f\in\mathcal{P}_k$, $S_tf=\bar{f}^\top e^{tA}b_k$, for all $t\ge0$.
\item $\mathcal{P}_k$ lies in the domain of $\mathcal{A}$ and $\mathcal{A}f\in\mathcal{P}_k$ for all  $f\in\mathcal{P}_k$.
\end{enumerate}
\end{theorem}
\begin{proof}
This theorem mirrors \citet{cuchiero2012polynomial} Theorem 2.7 in combinations with Remark 2.2 (ii).
\end{proof}

The existence of the linear map $A$ is convenient for moment calculation. The following corollary is useful for the construction of $A$ \citep[Equation 4.1]{cuchiero2012polynomial}.
\begin{corollary}\label{cor:poly}
Consider a $k$-polynomial process $X$ on $D$ with generator $\mathcal{A}$. Let $g_i\coloneqq e_i^\top  b_k$ be the $i$-th element of the polynomial basis, and let $h_i\coloneqq \mathcal{A}g_i=\bar{h}_i^\top b_k$. Construct the $N_k\times N_k$ matrix $A$ from $A_{ij}=\bar{h}_{i,j}$, then for all $f\in\mathcal{P}_m$, we have that $S_tf=\bar{f}e^{tA}b_k$ for all $t\ge0$.
\end{corollary}


